Iterative Reasoning Preference Optimization

Iterative preference optimization methods have recently been shown to perform well for general instruction tuning tasks, but typically make little improvement on reasoning tasks (Yuan et al., 2024, Chen et al., 2024). In this work we develop an iterative approach that optimizes the preference between competing generated Chain-of-Thought (CoT) candidates by optimizing for winning vs. losing reasoning steps that lead to the correct answer. We train using a modified DPO loss (Rafailov et al., 2023) with an additional negative log-likelihood term, which we find to be crucial. We show reasoning improves across repeated iterations of this scheme. While only relying on examples in the training set, our approach results in increasing accuracy on GSM8K, MATH, and ARC-Challenge for Llama-2-70B-Chat, outperforming other Llama-2-based models not relying on additionally sourced datasets. For example, we see a large improvement from 55.6% to 81.6% on GSM8K and an accuracy of 88.7% with majority voting out of 32 samples.

==> derivation.tex <==

\section{}

Let $y$ and $y'$ be two potential answers sampled from $p_{\theta}(\cdot | x)$ given a question or query $x$, with $p_\theta$ as the current, existing model parametrized by $\theta$. We assume access to $r^*(y,x)$ that allows us to tell which of these two answers, $y$ and $y'$, is better than the other. Without loss of generality, we say $r^*(y,x) > r^*(y',x)$. Then, the objective function for further improving the model, in terms of answer preferences, can be written down as
\begin{align}
    J(\theta) = -\mathbb{E}_{x \sim p_{\mathrm{data}}} \mathbb{E}_{y, y' \sim p_{\theta}(\cdot | x)}
    \underbrace{\log \left(1 + \exp \left(- \log \frac{p_\theta(y|x)}{p_{0}(y|x)} 
    + \log \frac{p_\theta(y'|x)}{p_{0}(y'|x)}\right)\right)}_{=-\mathcal{L}_{\mathrm{dpo}}},
\end{align}
where $\mathcal{L}_{\mathrm{dpo}}$ refers to the direct preference optimization~\citep{rafailov2023direct}.

To minimize this objective function, we resort to gradient-based optimization. We derive the per-example stochastic gradient as follows.
\begin{align}
    \nabla_{\theta} J(\theta; x)
    &=
    -\sum_{y, y'} \nabla_{\theta}\left[ p_{\theta}(y|x) p_{\theta}(y'|x) \log \left(1 + \exp \left(- \log \frac{p_\theta(y|x)}{p_{0}(y|x)} 
    + \log \frac{p_\theta(y'|x)}{p_{0}(y'|x)}\right)\right)\right] 
    \nonumber\\
    &=
    -\mathbb{E}_{y,y' \sim p_{\theta}(\cdot|x)} 
    \left[ 
    \log \left(1 + \exp \left(- \log \frac{p_\theta(y|x)}{p_{0}(y|x)} 
    + \log \frac{p_\theta(y'|x)}{p_{0}(y'|x)}\right)\right) \nabla_{\theta} \log p_{\theta} (y) 
    \right.
    \nonumber\\
    &\qquad
    +
    \log \left(1 + \exp \left(- \log \frac{p_\theta(y|x)}{p_{0}(y|x)} 
    + \log \frac{p_\theta(y'|x)}{p_{0}(y'|x)}\right)\right) \nabla_{\theta} \log p_{\theta} (y')
    \nonumber\\
    &\qquad
    \left.
    +
    \nabla_{\theta} \log \left(1 + \exp \left(- \log \frac{p_\theta(y|x)}{p_{0}(y|x)} 
    + \log \frac{p_\theta(y'|x)}{p_{0}(y'|x)}\right)\right)
    \right]
    \nonumber\\
    &\approx
    -\log \left(1 + \exp \left(- \log \frac{p_\theta(y|x)}{p_{0}(y|x)} 
    + \log \frac{p_\theta(y'|x)}{p_{0}(y'|x)}\right)\right) (\nabla_{\theta} \log p_{\theta}(y|x) 
    + \nabla_{\theta} \log p_{\theta}(y'|x) ) 
    \nonumber\\
    &\qquad
    -\nabla_{\theta} \log \left(1 + \exp \left(- \log \frac{p_\theta(y|x)}{p_{0}(y|x)} 
    + \log \frac{p_\theta(y'|x)}{p_{0}(y'|x)}\right)\right)
    \nonumber\\
    &=
    \mathcal{L}_{\mathrm{dpo}}(y, y', x) \nabla_{\theta} (\mathcal{L}_{\mathrm{NLL}}(y) + \mathcal{L}_{\mathrm{NLL}}(y'))
    + 
    \nabla_{\theta} \mathcal{L}_{\mathrm{dpo}}(y, y', x),
\end{align}
where we assume to use just a single pair of $(y, y')$ drawn from $p_{\theta}(y | x)$ to approximate the expectation. We use $\mathcal{L}_{\mathrm{NLL}}$ as a short hand of the negative log-probability

We emphasize three aspects of learning in this scenario based on this derivation. First, the answer pairs should be sampled from the current model, which makes it computationally challenging and also makes it more prone to high variance. We thus use the same set of samples drawn from the model for multiple gradient updates, assuming that a few updates, which we call collectively as an iteration, would not change the overall distribution $p_{\theta}$ too much. Second, we make the sampled answer pair to be more likely under the model, in addition to the more conventional direct preference loss. This ensures that in the next iteration the optimized pair is likely to be sampled again. After all, if the pair are not sampled again, it is a moot point to minimize the preference loss on this pair. This furthermore tells us that it is important to initialize $p_{\theta}$ to be reasonable. That is, an answer from this initial distribution must be good enough, if the goal is to sample an answer with a higher $r^*$. Finally, this derivation only works in a setting where we have access to $r^*$ such that we know which of the answers is preferred. There are cases, such as the one we explore in this paper, where this holds, but there are equally many cases where this does not hold, such as when expert annotation or costly experimentation is necessary to determine the preference between two answers.

From this objective function, we derive the practical and working algorithm, called \ourfullname{}. We describe this algorithm in detail in the next section. 

{\bf DPO SOLVED}


